Impedance Optimization for Uncertain Contact Interactions Through Risk Sensitive Optimal Control

This paper addresses the problem of computing optimal impedance schedules for legged locomotion tasks involving complex contact interactions. We formulate the problem of impedance regulation as a trade-off between disturbance rejection and measurement uncertainty. We extend a stochastic optimal control algorithm known as Risk Sensitive Control to take into account measurement uncertainty and propose a formal way to include such uncertainty for unknown contact locations. The approach can efficiently generate optimal state and control trajectories along with local feedback control gains, i.e. impedance schedules. Extensive simulations demonstrate the capabilities of the approach in generating meaningful stiffness and damping modulation patterns before and after contact interaction. For example, contact forces are reduced during early contacts, damping increases to anticipate a high impact event and tracking is automatically traded-off for increased stability. In particular, we show a significant improvement in performance during jumping and trotting tasks with a simulated quadruped robot.

==> sections/backup/02-contact_ocp.tex <==
% \section{Multi-Contact Robot Dynamics}\label{sec:muticontact_ocp}

% Robot dynamics in multi-contact scenarios can be described using 
% %
% \begin{align}
% \label{eqn:robot_dynamics}
%     M\left(q\right) \dot{v} + h\left(q,v\right)  = S^T \tau + J\left(q\right)^T \lambda_{ext} 
% \end{align}
% %
% % \noindent where, 
% % \footnotesize
% % \begin{align*}
% % &nj &&:\quad number\ of\ actuated\ joints \nonumber\\  
% % &nc &&:\quad number\ of\ active\ contacts \nonumber \\
% % &nq = nj + 7 &&:\quad dimension \ of \ configuration \ space \nonumber\\ 
% % &nv = nj + 6 &&:\quad dimension \ of \ tangent \ space \nonumber \\ 
% % &\tau \in R^m &&: \quad control\ inputs \nonumber \\ 
% % &q \in \mathcal{Q} \subseteq SE\left(3\right)\times R^{nj} &&: \quad element\ of\ configuration\ space \nonumber \\
% % &v \in \mathcal{T}_{q}\mathcal{Q} \subseteq R^{nv} &&: \quad element \ of  \ tangent \ space \ at \ q \nonumber \\ 
% % &\lambda_{ext} \in R^{6\times nc} &&: \quad active\ contact \ wrenches \nonumber 
% % \end{align*}
% % \normalsize
% %
% \noindent Where $q\in R^{nq}$ is the vector of generalized coordinates, $v\in R^{nv}$ is the vector of generalized velocities, $M\left(q\right)$ is the inertial matrix, $h\left(q,v\right)$ is the vector combining the nonlinear terms such as Coriolis acceleration and gravity, $S^T$ is the selection matrix mapping the controls to the actuated states, $\lambda_{ext}$ is the vector of contact forces and $J\left(q\right)$ is the contact Jacobian. The notation indicating the dependence on $q$ and $v$ will be omitted for the remainder of the text. The robot dynamics in~\eqref{eqn:robot_dynamics} can then be expressed as a first order differential equation
%  %
%  \begin{align}\label{eqn:first_order_dynamics}
%      \underbrace{\frac{d}{dt} \begin{bmatrix} q \\ v \end{bmatrix}  }_{\dot{x}} = \underbrace{ \begin{bmatrix} v \\ M^{-1} (\tau - h + J^T \lambda_{ext}) \end{bmatrix} }_{f(x, u)}
%  \end{align}
%  %
%  \noindent This defines the state vector as  $x^T=\left[q^T, v^T\right]\in \mathcal{X}$ the set of all possible states. Then the change in the state vector during a time interval $\delta t$ can be written as 
%  %
%  \begin{align}\label{eqn:motion_vector}
%      dx_t= \begin{bmatrix} dq_t \\ dv_t \end{bmatrix} = \delta t \begin{bmatrix} v_t \\ \dot{v}_t \end{bmatrix} = \delta t . f(x, u) % \in R^{2 nv}
%  \end{align}
% % 
% %  \noindent The motion vector is considered to live in the tangent space to the smooth manifold at a given state $x\left(t\right)$, hence $dx=\left[v, \dot{v}\right] \in \mathcal{T}_{x}\mathcal{X}$. The discrete first order dynamics then becomes 
%  %
%  \begin{align}\label{eqn:state_integration}
%     x_{t+1} = f_t\left(x_t,u_t\right) = x_t \oplus dx_t % = \begin{bmatrix}^bq_t \circ exp\left(^bdq_t\right) \\ ^jq_t + ^jdq_t \\ v_t + dv_t\end{bmatrix}
% \end{align}
% %
% \noindent where $\oplus$ handles the Lie group composition operation for the base orientation. Different contact models can be chosen to compute the contact forces $\lambda_{ext}$ \cite{stewart2000rigid,gilardi2002literature}.
 
%  \subsection{Rigid Contact Model}
% %
%  Let $p$, $\dot{p}$ and $\Ddot{p}$ denote any contact point position, velocity and acceleration respectively. During an active contact phase, the rigid contact assumption can be stated as
% %
% \begin{align}
%     \dot{p} &= J v = 0 \label{eq:rigid_contact_v}\\
%     \Ddot{p} &= \dot{J}v + J \dot{v} = 0\label{eq:rigid_contact_a}
% \end{align}
% %
% \noindent In order to resolve the contact forces for all active contacts, the robot dynamics~\eqref{eqn:robot_dynamics} is projected to the contact space using $\left(J M^{-1}J^T\right)^{-1} J M^{-1} = \Lambda  J M^{-1} $ to result in 
% %
% \begin{align}
%  \lambda_{ext} =   -\Lambda \dot{J}v + \Lambda J M^{-1} h - \Lambda J M^{-1} S^T \tau 
% \end{align}
% %
% \noindent Once $\lambda_{ext}$ is obtained, the motion vector~\eqref{eqn:motion_vector} can be constructed and the state vector $x_{t+1}$ can be obtained from~\eqref{eqn:state_integration}. 

 


% \subsection{Constrained Optimization of Multi-Contact Interactions}

% \quad The formulation presented above results in a predefined contact sequence upon which the considered dynamics model switches. Hence, at each contact switch the dimension of the contact space could change, leading to a change in the considered dynamics model. Given a predefined contact sequence, the cost function can be decomposed depending on the multi-contact phase specified and the optimal control problem is better expressed as  

% \begin{align}
%      \min_{\delta X,\delta U} &\quad l_T\left(\delta x_T\right) + \sum_{n=0}^{N} \sum_{t=0}^{T} l_t\left(\delta x_t, \delta u_t\right) \\
%      s.t. &\quad \delta x_{t+1} = f_n \left(\delta x_t, \delta  u_t\right)
% \end{align}

% \noindent where $N$ is the number of contact switches along along the trajectory and $T$ is the horizon of each phase. This model avoids the non-smooth switches in the contacts by solving the optimal control problem on multiple smooth intervals. The consistency at the transition between the switching intervals can be enforced through additional cost terms also known as soft constraints.   

% \noindent Moreover, friction cone constraints are added as soft constraints since the rigid contact model doesn't guarantee the unilateral nature of the contact forces or the Coulomb friction constraint. An inner square approximation of the cone constraint is considered and added as a cost term as done in~\cite{mastalli2019crocoddyl}, where the cost activates when the cone is violated, else it returns a zero cost. This is similar in spirit to handling contact  through relaxed log barrier functions~\cite{hauser2006barrier} however without the smoothing log barrier functions introduce. 

==> sections/backup/03-optimal_control.tex <==
% \section{Risk Sensitive Optimal Control}\label{sec:optimal_control}

% \quad In what is presented below we adopt the notation introduced in~\cite{dvijotham2012unifying} as it provides a unified formulation for the optimal control methods of interest. In general, an optimal control problem encompasses optimizing a  cost function as shown in~\eqref{Eq:functional} while being subject to the system dynamics in~\eqref{Eq:dynamics_sde} as well as other constraints. An optimal control solver then seeks to optimize a control policy $\pi\left(x_t\right)$ that drives the system dynamics along a trajectory $x\left(t\right)$ starting from an initial condition $x\left(0\right)$ while minimizing a cost similar to~\eqref{Eq:stoch_ocp_cost}.  

% \begin{align}
%     \mathcal{J}^{*}\  &= \min_{\pi\left(x_t\right)}\quad   \Psi_{\pi\left(x_t\right)}^{\sigma} \left[\mathcal{L}\left(x,\pi\left(x\right)\right)\right]   \label{Eq:stoch_ocp_cost}\\
%     \textrm{s.t.}\   &   dx_t = f\left(x_t,u_t\right) dt + F\left(x_t,u_t\right) d\omega_t \label{Eq:dynamics_sde} \\ 
%     \textrm{where} \  & \mathcal{L}\left(x,\pi\left(x\right)\right) = l_T\left(x_T\right) + \sum_{0}^{T-1} l_t\left(x_t,\pi\left(x_t\right)\right) \label{Eq:functional} \\
%     & \quad \Psi_{\pi\left(x_t\right)}^{\sigma} \left[\mathcal{L}\right] = \frac{1}{\sigma} \log\left(\mathbb{E}\left[\exp{\left(\sigma \mathcal{L}\right)}\right] \right) \label{Eq:risk_cost}
% \end{align}

% \noindent Where $f\left(x_t, u_t\right)$ is the drift term of the system dynamics and $F\left(x_t, u_t\right)$ is the diffusion term associated with the Brownian motion $d\omega_t$. The cost function $l_t\left(x_t,\pi\left(x_t\right)\right)$ is used to describe a desired behavior or task for the robot such as the center of mass motion or the contact forces desired at the end effectors at a certain instant $t$ in time. Then, $\Psi_{\pi\left(x_t\right)}^{\sigma} \left[\mathcal{L}\right]$ is a transformation of the original cost functional $\mathcal{L}\left(x,\pi\left(x\right)\right)$ and is described in~\eqref{Eq:risk_cost} where $\mathbb{E}\left[\boldsymbol{\cdot} \right]$ is the expectation and $\sigma$ is a scalar known as the sensitivity parameter. Considering the first order approximation of~\eqref{Eq:risk_cost} provides an insight to the generalization this formulation provides. This approximation is derived in details in~\cite{farshidian2015risk} and presented in~\eqref{Eq:cost_approximation}. 

% \begin{align}
%     \Psi_{\pi}^{\sigma} \left[\mathcal{L}\left(x,\pi\right)\right] \approx \mathbb{E}_{\pi}\left[\mathcal{L}\left(x,\pi\right)\right] + \sigma \mathbf{Var}\left[\mathcal{L}\left(x,\pi\right)\right] \label{Eq:cost_approximation}
% \end{align}

% \noindent Having a positive sensitivity parameter $\sigma > 0$ means that a higher variance accumulates more cost, thus an optimizer would seek a solution minimizing the variance in order to further minimize the cost. It was shown in~\cite{jacobson1973optimal} that as $\sigma \to + \infty$ the solution converges to that of $H^\infty$ control for the linear case, Campi~\cite{campi1996nonlinear} discussed the limits presented for the nonlinear case. For the case where  $\sigma < 0$,  the higher the variance is the lower the cost is, hence an optimizer would prefer a risk seeking behavior. Risk seeking behavior is not a common setting in the control of robotics and is rather used as a method to facilitate exploration for reinforcement learning algorithms~\cite{bechtle2020curious}. In the limit as $\sigma \to 0$ the optimal solution converges to that of minimizing the expectation only, also known as the linear quadratic regulator LQR.  

% To avoid the curse of dimensionality associated with feedback optimal control problems, few restrictive assumptions have to be made. The feedback control law is restricted to linear feedback in the states $ \pi\left(x\right) = \tau + K_{fb} \delta x $. Mayne~\cite{mayne1966second} developed a local iterative scheme to handle nonlinear dynamics and cost functions around a nominal state and control trajectories denoted $\mathcal{X}^n=\{x^n_0, x^n_1, ..., x^n_N\}$ and  $\mathcal{U}^n=\{u^n_0, u^n_1, ..., u^n_{N-1}\}$ respectively. The solution to the finite horizon stochastic optimal control problem can be obtained recursively using the Extended Hamilton Jacobi Bellman equations for the nonlinear risk sensitive case as described in~\cite{farshidian2015risk}.

% \subsection{Cost Function and Process Model Approximations}

% \quad The deviations from the nominal trajectories are simply defined as, 
% \begin{align}
%     \delta x_t = x_t - x^n_t, \quad \quad \delta u_t = u_t - u^n_t
% \end{align}

% A local linear approximation of the system dynamics and a quadratic approximation of the cost function can be constructed with respect to the same state and control deviations as, 

% \begin{align}
%     %\mathcal{L}\left(\delta x_t, \delta u_t\right) =& l_N\left(\delta x_N\right) + \sum_{t=0}^{N-1} l_t\left(\delta x_t, \delta u_t\right) \\ 
%     \delta x_{t+1} =& A_t \delta x_t + B_t \delta u_t + C_t  \omega_t \\
%     l_t\left(\delta x_t, \delta u_t\right) =& \delta x_t^T Q_t \delta x_t + \delta x_t^T q_t + q_t^0 \\
%     &+ \delta u_t^T R_t \delta u_t + \delta u_t^T r_t + r_t^0  \nonumber \\
%     where \quad A_t &= dt.\frac{\partial f}{\partial x}\bigg\vert_{x^n_t,u^n_t} \quad B_t = dt.\frac{\partial f}{\partial u}\bigg\vert_{x^n_t,u^n_t}  \\  \quad C_t &= \sqrt{dt}.F\bigg\vert_{x^n_t,u^n_t} \nonumber 
% \end{align}
% % \noindent Then the linear approximation of the system dynamics and the quadratic approximation of the cost can be derived in terms of the deviations in discrete time as 
% %  \begin{align}
% %     %\delta x_{t+1} =& A_t \delta x_t + B_t \delta u_t + C_t  \omega_t \\  
    
% % \end{align}

% \noindent $Q_t , \ R_t, \ q_t , $ and $r_t$ are the respective hessians and gradients of the cost function with respect to the states and controls. The cross term relating the dynamics and controls is omitted for brevity of description. For the deterministic case, or the case where $C_t$ is not state or control dependent and the noise is Gaussian $\omega_t \sim \mathcal{N}\left(0, \Omega \right)$, the optimal control solution turns out to be the same. This is known as the Certainty Equivalence principle. 
% % In~\cite{todorov2005generalized} Gaussian process noise of multiplicative nature is considered. Under such assumption, the certainty equivalence principle doesn't hold anymore, and the optimal control solution is a function of the process noise expectation in the value function. This naturally leads to stiff control policies that aggressively counter any process disturbances along the trajectory. 

% \subsection{Feedback as a Function of Measurement Uncertainty}

% \quad In order to include measurement uncertainty, Speyer~\cite{speyer1974optimization} had to introduce a state vector that grows at each time step to include the entire observed state history. Ponton~\cite{ponton2020effects} suggested that doubling the size of the state vector to include the dynamics of an Extended Kalman Filter eliminates the need for a growing state vector providing an efficient and tractable risk sensitive control algorithm that accounts for the uncertainty in both the process and measurements. To summarize the results developed by Ponton, consider the general measurement model 
% \begin{align}
%     dy_t = h\left(x_t,u_t\right) dt + H\left(x_t,u_t\right)d\gamma\label{Eq:measurement_model}
%  \end{align}

% \noindent where $\gamma_t \sim \mathcal{N}\left(0, \Gamma \right)$. Assuming an observable system, an Extended Kalman Filter can be used to compute the estimate deviations $\delta \hat{x}_t$ along the nominal trajectory $\mathcal{X}^n$ at each iteration. The extended system dynamics then become 

% \begin{align}
%     \begin{bmatrix} d\left(\delta x_t\right) \\ d\left(\delta \hat{x}_t\right) \end{bmatrix} =& \begin{bmatrix}A_t\delta x_t + B_t \delta u_t \\ A_t\delta x_t + B_t \delta u_t + K_t F_t \left(\delta x_t - \delta \hat{x}_t\right) \end{bmatrix}dt  \nonumber \\ &+ \begin{bmatrix} C_t & 0  \\ 0 & K_t D_t \end{bmatrix} \begin{bmatrix}d\omega_t \\ d\gamma_t \end{bmatrix}
% \end{align}

% \noindent where $F_t$ and $D_t$ are the local approximations of $h\left(x_t,u_t\right)$ and $H\left(x_t,u_t\right)$ respectively. At each iteration, the  estimator gains $K_t$ are computed along the nominal trajectory, then the optimal control law is optimized through solving the value function recursively. As before with accounting for the process uncertainty, a higher process noise results in stiff policies that drive the system robustly along the desired trajectory. However, taking the measurement uncertainty into consideration brings a new advantage, that is,  an increase in the compliance of the controller in response to the increase in the measurement uncertainty. A natural result as aggressive control responses are not favorable under uncertain measurement scenarios. The solution to the risk sensitive optimal control problem with measurement uncertainty is presented in \cite{ponton2020effects}.



% \subsection{Error State Kalman Filter on Smooth Manifolds}

% \quad A full state measurement model is considered to construct the estimator. The estimation error $\delta x$ is defined on the tangent space $\mathcal{T}_{x}\mathcal{X}$ so is its covariance~\cite{sola2018micro}. The error in the state and its covariance can then be represented as 

% \begin{align}
%     \delta x &= x \ominus \hat{x}  \\ % = \begin{bmatrix} log\left(^b\hat{q}^{-1}\circ ^bq\right) \\ ^j\hat{q} - ^jq \\ \hat{v} - v\end{bmatrix} \in R^{2 nv}
%     \Sigma &= \mathbb{E}\left[\delta x . \delta x^T \right] %\in R^{2 nv \times 2 nv}
% \end{align}

% \noindent Where $\ominus$ represents the difference between the two states $\hat{x}$ and  $x$ with the proper Lie group operations~\cite{sola2018micro}. The gaussian noise $\varepsilon \sim \mathcal{N}\left(0, \Sigma\right)$ is then defined on the same space as the estimation error, and the covariance can be propagated through the adjoint transformation while the state prediction follows the relative group composition operation described earlier in~\eqref{eqn:state_integration}. 
% \begin{align}
% \Sigma_{t+1} &= Ad_{dx} \Sigma_{t} Ad_{dx}^T + \Omega_{t+1} 
% \end{align}

% A full treatment of Extended Kalman Filters on lie groups can be found in  ~\cite{sola2018micro},~\cite{blanco2010tutorial} and~\cite{sola2017quaternion}.%Various numerical methods of implementing an Extended Kalman Filter along with the detailed theory is provided in~\cite{bar2004estimation}.



% \subsection{Constrained Optimization of Multi-Contact Interactions}

% \quad The formulation presented above results in a predefined contact sequence upon which the considered dynamics model switches. Hence, at each contact switch the dimension of the contact space could change, leading to a change in the considered dynamics model. Given a predefined contact sequence, the cost function can be decomposed depending on the multi-contact phase specified and the optimal control problem is better expressed as  

% \begin{align}
%      \min_{\delta X,\delta U} &\quad l_T\left(\delta x_T\right) + \sum_{n=0}^{N} \sum_{t=0}^{T} l_t\left(\delta x_t, \delta u_t\right) \\
%      s.t. &\quad \delta x_{t+1} = f_n \left(\delta x_t, \delta  u_t\right)
% \end{align}

% \noindent where $N$ is the number of contact switches along along the trajectory and $T$ is the horizon of each phase. This model avoids the non-smooth switches in the contacts by solving the optimal control problem on multiple smooth intervals. The consistency at the transition between the switching intervals can be enforced through additional cost terms also known as soft constraints.   

% \noindent Moreover, friction cone constraints are added as soft constraints since the rigid contact model doesn't guarantee the unilateral nature of the contact forces or the Coulomb friction constraint. An inner square approximation of the cone constraint is considered and added as a cost term as done in~\cite{mastalli2019crocoddyl}, where the cost activates when the cone is violated, else it returns a zero cost. This is similar in spirit to handling contact  through relaxed log barrier functions~\cite{hauser2006barrier} however without the smoothing log barrier functions introduce. 

==> sections/backup/contact_impedance.tex <==
\section{Response Due to Unexpected Contact}

transform the impedance into some frame space, either contact or CoM , will give us an idea how to contact point will behave due to unexpected early contact force,  \textcolor{red}{does it make sense to study frequency response of the z position of contact point due to unexpected contact force?} 

\begin{align}
    \Lambda \delta \Ddot{x} + Kd_{ee} \delta \Dot{x} + Kp_{ee} \delta x = \lambda  
\end{align}

\noindent where $J^\dagger = J^T \left(J J^T\right)^{-1}$ is the pseudo inverse of the jacobian of the space we wish to study the impedance in, note that a contact force must be transferred to the same space (CoM impedance study for example).  

\begin{align}
    \Lambda  &= \left(J M^{-1} J^T\right)^{-1} \\ 
    Kp_{ee} &= \Lambda JM^{-1} S^T K_{q} J^\dagger \\ 
    Kd_{ee} &= \Lambda JM^{-1} S^T K_{\dot{q}}J^\dagger
\end{align}

\noindent \textcolor{red}{From Ludo: your computation gives you the contribution to the impedance due to the dx displacement - but you have another part that comes from the displacement in the nullspace of  dx that will change the impedance at the leg... this is because you multiply dq by K}

==> sections/backup/contact_uncertainty.tex <==
\section{Uncertainty in Contact Interactions}

One way to model uncertainty in contact location is to extend the state vector to include the contact position. Another way is to model this uncertainty as uncertainty in the swing foot position and transform it back to the full body measurement model \textcolor{red}{needs paraphrasing}. To do so, start by expressing the error in the end effector position in terms of the state vector. 

\begin{figure}[h]
\centering
  \includegraphics[width=.8\linewidth]{figures/ellipse_noFrame.png}
  \caption{Uncertainty ellipsoid reaching contact before mean}
  \label{fig:contact_uncertainty}
\end{figure}


\subsection{Extended Kalman Filter on Smooth Manifolds}
Full state measurement, state vector is not extended by any extra states. \cite{carpentier2019pinocchio} and \cite{rotella2014state}, since the robot dynamics evolve on a smooth manifold instead of a vector space, care must be taken when defining uncertainty and constructing the Extended Kalman Filter - \textit{EKF}. The estimation error $\delta x$ is defined on the tangent space $\mathcal{T}_{x}\mathcal{X}$ so is its covariance  
\begin{align}
    \delta x &= x \ominus \hat{x} \in R^{2 nv}\\
    \Sigma &= \mathbb{E}\left[\delta x . \delta x^T \right] \in R^{2 nv \times 2 nv}
\end{align}

\noindent The gaussian noise $\varepsilon \sim \mathcal{N}\left(0, \Sigma\right)$ is defined on the same space as the estimation error, hence $\varepsilon \in \mathcal{T}_x\mathcal{X}$
\begin{align}
\Sigma_{t+1} &= Ad_{x_r} \Sigma_{t} Ad_{x_r}^T + \Omega_{t+1} \\ 
x_r &= exp\left(dx_t\right) \nonumber 
\end{align}
This is mainly from \cite{sola2018micro}, \cite{blanco2010tutorial} and \cite{sola2017quaternion}, since we are using a full state measurement model, the measurement uncertainty can be propagated the same way. Once the transitions and spaces are defined properly, the estimation algorithm follows that of the well known extended kalman filter, \cite{bar2004estimation}.




\subsection{Uncertainty in the Contact}\label{sec:contact_uncertainty}

any frame is defined as SE(3) element, noise is defined on the tangent space to this element locally. uncertainty in the contact locations is defined in the global frame, hence we first need to transform it to the local frame through $Ad^{-1}$. This is a well defined affine transformation, hence  using the affine property of Gaussians, we can transform the uncertainty to the tangent space at a given point in SE(3). let $x \sim \mathcal{N}(\mu,\,\Sigma)$ be a Gaussian random variable, and $f(x)= Ax + b$ be an affine transformation, then the transformation gives a Gaussian random variable  $f(x) \sim \mathcal{N}(A \mu + b,\,A \Sigma A^T) $. We will use this property at two stages, first the transformation to the local frame error, second when transforming to the configuration space \cite{sola2018micro}. Note properties of linear transformations of Gaussians and their covariance. An error in the position is transformed like a velocity vector 
whereas an error in the velocity is transformed like an acceleration. Finally use the jacobian to transform the position and velocity error to the configuration space through the Moore-Penrose inverse 

\begin{align} \label{eqn:rigid_contact_model}
    \begin{bmatrix} \Dot{x} \\ \Ddot{x} \end{bmatrix} = \underbrace{\begin{bmatrix} J & 0 \\ \Dot{J} & J \end{bmatrix}}_{A} \begin{bmatrix} \Dot{q} \\ \Ddot{q} \end{bmatrix}   
\end{align}

\noindent Then the errors can be expressed as 

\begin{align}
    \begin{bmatrix} \delta q \\ \delta \dot{q} \end{bmatrix}   =A^{\dagger} \begin{bmatrix} \delta x \\ \delta \dot{x} \end{bmatrix} \label{eqn:contact_uncertainty_model}
\end{align}

\noindent Where $A^{\dagger}$ is the Moore-Penrose inverse defined as $A^{\dagger} = A^T \left(A.A^T\right)^{-1}$. Now the errors are in the same vector space as the full state noise, what remains is projecting the noise to the null space of the active contacts to be consistent with the optimization model, the contact constraint can be defined similarly as \eqref{eqn:rigid_contact_model}, let $J_c$, $\dot{J}_c$ and $A_c$ be the respective matrices. The null space projection can be defined as 

\begin{align}
    P_c = I - A_c^\dagger A_c 
\end{align}

and the contact noise effect can be written as 

\begin{align}
    \begin{bmatrix} \delta q \\ \delta \dot{q} \end{bmatrix}   =\left(I - A_c^\dagger A_c\right) A^{\dagger} \begin{bmatrix} \delta x \\ \delta \dot{x} \end{bmatrix} \label{eqn:contact_uncertainty_model}
\end{align}



\subsection{Effect on the Full State Uncertainty}

take different configurations of the swing foot, how far are we from the contact and does this map to the full state  covariance matrix, measurement noise will then project to the full state measurement noise as, 

\begin{align}
    \Gamma = \Gamma_{fs} + P_c A^{\dagger} \Gamma_{c} A^{\dagger^T} P_c^T
\end{align}

\noindent Where $\Gamma_{fs}$ denotes the full state noise while. $\Gamma_{c}$ denotes the noise in the contact space or end effector space. Here we will study how the structure of the uncertainty matrix changes as a function of the configuration and the noise model used. This will help in relating it to the feedback matrix structure obtained later. 

\begin{figure}[h]
\centering
  \includegraphics[width=.75\linewidth]{figures/uncertainty/contact_jacobian.pdf}
  \caption{Uncertainty with no contact constraints}
  \label{fig:uncertainty_jacobian}
\end{figure}

\begin{figure}[h]
\centering
  \includegraphics[width=.75\linewidth]{figures/uncertainty/contact_consistent.pdf}
  \caption{Contact consistent uncertainty}
  \label{fig:uncertainty_contact}
\end{figure}

\noindent \textcolor{red}{Projecting the swing foot noise onto the null space of the active contact constraints has a significant effect of the structure of the matrix.} \textcolor{blue}{Where would it make sense to have higher values, swing positions, or swing velocities?} 


\section{Extensions and Improvements}

things that I would like to improve before sending this anywhere 

\begin{itemize}
    \item inject and filter joint noise  
    \item convergence and quantifying noise effect on the stability of the algorithm \cite{sideris2005efficient} and \cite{roulet2019convergence}
    \item different measurement model that reason about contact \cite{hartley2020contact},  \cite{hertzberg2013integrating} and \cite{rotella2014state}
    \item better cost function that reasons about contact forces and control frequency \cite{grandia2019frequency}, \cite{grandia2019feedback}
    \item impedance analysis/stability \cite{boaventura2015model}, \cite{geoffroy2014two}, \cite{aghasadeghi2013learning}
    \item optimize a jump, \cite{ponton2018time} 
    \item possibility of running an experiment ? 
\end{itemize}



==> sections/backup/experiments.tex <==
\section{Results}

The experiments in this section will be using a version of the quadruped robots introduced in \cite{grimminger2019open}. A single step with applying force task will be first presented with the full analysis, then the same approach will be used to demonstrate a trot gait with unexpected contacts.  For generating reference trajectories for the controller around which the local controller is computed, we use the kino-dynamic optimizer described in \cite{ponton2018time}. 

\noindent All dynamics computations and their derivatives are carried out using \textit{pinocchio} dynamics library \cite{carpentier2019pinocchio}. The library is also used to simulate the robot with a linear soft contact model. % of the form 
% \begin{equation}
%     \lambda_{contact} = k \left(x_{ref}-x_{contact}\right) - b \Dot{x}_{contact}
% \end{equation}
\noindent Simulation steps are computed at $dt_{sim} = 1.e{-5}\ sec$ with  stiffness parameter of $k=1.e{+5}$ and a damping parameter of $2.e{+2}$. The friction coefficient used in simulation is $\mu = 0.7$. The control loop is computed at a period of $dt_{control} = 1.e{-3} \ sec$, hence the control is run at a $1kHz$ frequency. The trajectory and control optimization is computed at a time step $dt_{opt} = 1.e{-2} \ sec$ and then the computed trajectory is interpolated for 10 steps to match the control frequency. The sensitivity parameter is set to $s =\ 5$ for both experiments. 

\subsection{Experiment 01}



\noindent In this experiment, the task is to swing a single leg \textit{FL} for a maximum height of $10\ cm$ and a distance of $8\ cm$ . Unexpected contact occurs at $3\ cm$ higher than the optimized  trajectory $~ 9.2\%$ of the total leg length. The purpose of this experiment is to demonstrate the effect of different ways of modeling contact uncertainty on the feedback gains and impact forces. 
The task is divided into 4 phases, namely  full support \textit{FS} where all feet are on the ground, swing phase \textit{SP} where multiple feet could break contact with the ground while at least one keeps contact, switch phase \textit{SW} where a certain foot is approaching a contact surface, and back to full support \textit{FS}. The task cost function could then be written as follows, 
\begin{align}
    L &= \sum_{t=0}^{t=10} L_{FS} + \sum_{t=10}^{t=50} L_{SP}+ \sum_{t=50}^{t=55} L_{SW} + \sum_{t=55}^{t=65} L_{FS}
\end{align}

\begin{figure}[h]
\centering
\subfloat[][Position error norm]{
\includegraphics[width=0.23\textwidth]{results/single_step/exp01_qerror.pdf}
\label{fig:exp01_feedback_ddp}}
% \qquad
\subfloat[][Velocity error norm]{
\includegraphics[width=0.225\textwidth]{results/single_step/exp01_dqerror.pdf}
\label{fig:exp01_feedback_rs_state}} \\
\subfloat[][Stiffness norm]{
\includegraphics[width=0.23\textwidth]{results/single_step/exp01_kp.pdf}
\label{fig:exp01_feedback_rs_joints}}
% \qquad
\subfloat[][Damping norm]{
\includegraphics[width=0.225\textwidth]{results/single_step/exp01_kd.pdf}
\label{fig:exp01_feedback_rs_jacobian}}
\caption{Feedback at time of unexpected impact t = 0.43 sec}
\label{fig:exp01_feedback_compare}
\end{figure}

\noindent The impedance profile is then optimized for the finite horizon problem along with the state and control trajectories using DDP and the risk sensitive formulation with measurement noise. Three different types of measurement noise models are used. uniform full state measurement noise, noise added to the joints of the swing leg only, and swing leg noise mapped back to the full state noise using \eqref{eqn:contact_uncertainty_model}. The effect of the measurement noise model used is depicted in fig. \ref{fig:exp01_feedback_compare}. A uniform noise at the full state measurement produces a reduced intensity feedback fig. \ref{fig:exp01_feedback_rs_state} compared to that of DDP fig. \ref{fig:exp01_feedback_ddp} while keeping the same structure. Modeling a higher uncertainty on the joint positions and velocities of the swing foot shifts the feedback to the feet positions mostly, hence increasing the stiffness of the legs fig. \ref{fig:exp01_feedback_rs_joints}, this is an undesired behavior in impedance control while approaching a contact with an uncertain position. Using the method described in \ref{sec:contact_uncertainty} yields higher damping gains on the joints of the legs and a higher stiffness on the base position fig. \ref{fig:exp01_feedback_rs_jacobian}. 


\begin{figure}[h]
\centering
\subfloat[][kp DDP]{
\includegraphics[width=0.225\textwidth]{results/single_step/ddp_kp.pdf}
\label{fig:exp01_feedback_ddp}}
% \qquad
\subfloat[][kd DDP]{
\includegraphics[width=0.225\textwidth]{results/single_step/ddp_kd.pdf}
\label{fig:exp01_feedback_rs_state}} \\
\subfloat[][kp RS swing joints]{
\includegraphics[width=0.225\textwidth]{results/single_step/joint_kp.pdf}
\label{fig:exp01_feedback_rs_joints}}
% \qquad
\subfloat[][kd RS swing joints]{
\includegraphics[width=0.225\textwidth]{results/single_step/joint_kd.pdf}
\label{fig:exp01_feedback_rs_jacobian}}\\
\subfloat[][kp RS unconstrained]{
\includegraphics[width=0.225\textwidth]{results/single_step/unconstrained_kp.pdf}
\label{fig:exp01_feedback_rs_joints}}
% \qquad
\subfloat[][kd RS unconstrained]{
\includegraphics[width=0.225\textwidth]{results/single_step/unconstrained_kd.pdf}
\label{fig:exp01_feedback_rs_jacobian}}\\
\subfloat[][kp RS constrained]{
\includegraphics[width=0.225\textwidth]{results/single_step/null_kp.pdf}
\label{fig:exp01_feedback_rs_joints}}
% \qquad
\subfloat[][kd RS constrained]{
\includegraphics[width=0.225\textwidth]{results/single_step/null_kd.pdf}
\label{fig:exp01_feedback_RS}}
\caption{Feedback at time of unexpected impact t = 0.43 sec}
\label{fig:exp01_feedback_compare}
\end{figure}

\noindent The effect of the optimized impedance profile using risk sensitive control with contact uncertainty is compared to that of DDP through a simulation with an unexpected $3\ cm$ contact occurring at time  $t=\ 0.43\ sec$. The contact forces are shown in fig. \ref{fig:exp01_contact_force}. \textit{FL} being the swing foot, using the gains computed with risk sensitive, the impact force is lower, moreover, contact force tracking at the support feet \textit{FR}, \textit{HL}, and \textit{HR} is significantly better, while the error due to the unexpected impact force causes the contact forces on the support feet to deviate.  

\noindent The tracking behavior of both controllers is presented in fig. \ref{fig:exp01_errors_gains}. The state-error $\delta x$ is divided into position and velocity errors $\delta q$ and $\delta \dot{q}$ respectively. The feedback gain matrix is divided into two parts, $K_p$ and $K_d$ where they multiply $\delta q$ and $\delta \dot{q}$ respectively representing the stiffness and damping of the full state vector. The vector norm $\Vert v \Vert =  \sqrt{v^T.v}$ is used to compute the error norms whereas the Frobenius Norm $\Vert M \Vert_F = \sqrt{Tr\left(A.A^T\right)}$ is used to compute the feedback norms. From fig. \ref{fig:exp01_kp_norm} it is clear that the DDP computed stiffness is orders of magnitude higher than that of risk sensitive $\frac{\vert K_p\vert_{DDP}}{\vert K_p\vert_{RS}} \approx  \frac{1500}{20}$ at its peak. While the norm of the damping part of the matrix $\frac{\vert K_d\vert_{DDP}}{\vert K_d\vert_{RS}} \approx  \frac{40}{10}$. Another way of seeing the difference $\vert K_p\vert_{DDP} \approx 20 \vert K_d\vert_{DDP}$ while $\vert K_p\vert_{RS} \approx 2 \vert K_d\vert_{RS}$.  



\noindent This reflects significantly on the tracking performance of the controller in simulation. At impact time $r=\ 0.43\ sec$ the position error $\delta q$ shown in fig. \ref{fig:exp01_qerror} rises due to the higher contact position, in the case of RS it stabilizes while it clearly diverges for DDP. The effect is more clear in fig. \ref{fig:exp01_dqerror} where a spike in the velocity error occurs, while RS manages to dam it back, DDP fails as it keeps rising. 


\noindent \textcolor{red}{Is it actually better than full state noise?} Below is a gain matrix at $t=0.43 \ sec$ along with the covariance, contact forces and feet height 



\begin{figure}[h]
    \centering
  \includegraphics[width=.9\linewidth]{results/one_step/contact_force_z.pdf}
  \caption{Normal force for quadruped feet}
  \label{fig:exp01_contact_force}
\end{figure}


% \begin{figure}[h]
%     \centering
%   \includegraphics[width=.9\linewidth]{results/one_step/feet_height.pdf}
%   \caption{Normal force for quadruped feet}
%   \label{fig:exp01_contact_height}
% \end{figure}





\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{results/exp02/trot_sim03.pdf}
\caption{Trotting Gait}
\end{figure*}

\subsection{Experiment 02 - A Trotting Gait}

The purpose of this experiment is to show how risk sensitive control with measurement uncertainty out performs DDP by simulating a $3 \ sec$ trotting trajectory. Two $3 \ cm$ high blocks are added to the simulation as unexpected contact disturbances. While DDP fails after the first disturbance, the controller computed using risk sensitive control survives both disturbances without the need to recompute trajectories in a model predictive control fashion. 

\noindent Fig. \ref{fig:exp02_contact_feet_tracking} depicts the tracking performance of the feet height. Stepping on a higher object occurs for the swing leg $FL$ at $ 0.8\ sec \leq t \leq  1.35 \sec$, once the opposing leg  $FR$ takes of the ground, DDP fails at maintaining the desired contact force while RS performance is not affected. The second interesting behavior is at $t=1.6\ sec$ where a delayed contact occurs because of stepping from a higher surface to a lower one. The corresponding normal force to this delayed contact regulated back to achieve a good tracking as shown in fig. \ref{fig:exp02_contact_force}.  


\begin{figure}[h]
\centering
  \includegraphics[width=.9\linewidth]{results/exp02/feet_height.pdf}
  \caption{Trot Gait feet height with obstacles}
  \label{fig:exp02_contact_feet_tracking}
\end{figure}

\begin{figure}[h]
\centering
  \includegraphics[width=.9\linewidth]{results/exp02/normal_force.pdf}
  \caption{Trot Gait Normal Force}
  \label{fig:exp02_contact_force}
\end{figure}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth]{results/exp02/trot_sim.pdf}
% \caption{Trotting Gait}
% \end{figure*}


==> sections/backup/impedance_control.tex <==
\section{Impedance Control}
\textcolor{red}{Here I discuss basic impedance control and tools that could be useful in studying the performance of these controllers}

\noindent A second order system step response study could be useful as suggested by \cite{park2012impedance}. Where as Poincar\`{e} maps and bifurcation analysis is used in \cite{lee2014dynamics} and \cite{kronander2016stability} devises a Lyapunov function to study the stability of changing impedance along a trajectory.    
\noindent The impedance control law in tasks space is given by 

\begin{align}
    M_e d\Ddot{x} + B_e \dot{x} + K_e dx = \lambda_{ext}
\end{align}

\subsection{Stability in Impedance Control}

\noindent Here's how to study if the gains generated could make sense in terms of impedance control, simply start by replacing the feedback law 



\begin{align}
    M \Ddot{q} + h\left(q,\dot{q}\right)  = S^T \left(\tau_{ff} +K_{q} \delta q +  K_{\Dot{q}} \delta \dot{q}\right) + J^T \lambda_{ext} \\ 
\end{align}

\noindent We can use the least squares solution to write the joint velocities as a function of the frame velocities. 
\begin{align}
    \delta q &= J^T \left(J J^T\right)^{-1} \delta x \\
    \delta \dot{q} &= J^T \left(J J^T\right)^{-1} \delta \dot{x}
\end{align}
\noindent Now we want to transform the robot dynamics to the contact space to study the effect of an input force on the entire system. To do so, we start by describing the desired frame motion 

\begin{align}
    \dot{x} &= J \dot{q} \\
    \Ddot{x} &= \dot{J}\dot{q} + J \Ddot{q}
\end{align}

\noindent Then multiplying by $JM^{-1}$ we can replace back the frame acceleration to get 

\begin{align}
    \Ddot{x} - \dot{J}\dot{q}  &+ JM^{-1} h\left(q,\dot{q}\right) = JM^{-1} S^T \tau_{ff} \nonumber \\
    &+ JM^{-1} S^T K_{q} J^T \left(J J^T\right)^{-1} \delta x \nonumber \\
    &+ JM^{-1} S^T K_{\dot{q}} J^T \left(J J^T\right)^{-1} \delta \dot{x} \nonumber \\
    &+ JM^{-1}J^T \lambda_{ext}
\end{align}

 
\noindent Where $K_{q}$ is the block of the feedback matrix that multiplies the position errors, and $K_{\Dot{q}}$ is the block multiplying the velocity error. We can multiply the whole system with the end-effector inertia given by 

\begin{align}
    \Lambda\left(q\right) = \left(J M^{-1}J^T\right)^{-1}
\end{align}

This results in a second order system dynamics of the form presented in \eqref{eqn:contact_space_impedance}, note that all contact forces at all end effectors must be transformed to the desired frame using the appropriate transformations. 

\begin{align}
    \Lambda\left(q\right) \delta \Ddot{x} + Kd_{ee}\delta \dot{x} + Kp_{ee}\delta x = \lambda_{ext} \label{eqn:contact_space_impedance}
\end{align}

Now we have the robot dynamics expressed as second order dynamics in the contact space including the feedback law. 
This would allow us to study the response of the system due to an impact force. This means we have the stiffness and damping of the end-effector when the controller is applied as follows 

\begin{align}
    Kp_{ee} &= \left(J M^{-1}J^T\right)^{-1}JM^{-1} S^T K_{q} J^T \left(J J^T\right)^{-1}\\ 
    Kd_{ee} &= \left(J M^{-1}J^T\right)^{-1}JM^{-1} S^T K_{\dot{q}} J^T \left(J J^T\right)^{-1}
\end{align}

\noindent \textcolor{red}{From Ludo: your computation gives you the contribution to the impedance due to the dx displacement - but you have another part that comes from the displacement in the nullspace of  dx that will change the impedance at the leg... this is because you multiply dq by K}



% \subsection{Alternative Derivation}

% From \cite{murray2017mathematical} we know that 

% \begin{align}
%     Kp_{q} &= J^T Kp_{x} J \\ 
%   \left(JJ^T\right)^{-1} J Kp_{q} &=  Kp_{x} J \\
%   \left(JJ^T\right)^{-1} J Kp_{q} J^T &=  Kp_{x} J J^T \\
%   \left(JJ^T\right)^{-1} J Kp_{q} J^T \left(JJ^T\right)^{-1} &=  Kp_{x}
% \end{align}

\noindent \textcolor{blue}{All other impedance control approaches design the gains in task space then feed the outcome to an inverse dynamics controller. What advantage do we get in designing the impedance in the joint space? Why does it make sense to do the feedback on the full body model?}

==> sections/backup/introduction.tex <==
\section{Introduction}

Interacting with the environment would require a robot to establish and break contact multiple times to achieve a given task. During these contact interactions a robot would exert forces on the environment in order to either move an object, or use the generated forces to move itself around. Thus, robots must be able to generate and track a set of desired forces at certain contact locations in the environment in order to accomplish a desired task. However, intermittent contacts increase drastically the complexity of the control design problem if approached with classical control design techniques. One challenge arises during contact switching events, such events are typically characterized by their abrupt and stiff nature. Impact forces resulting from contact switches usually lead to high disturbances and instantaneous changes in a robot's motion. Another major challenge occurs when a robot miss-estimates a contact location accurately. In an ideal world where the robot's perception of itself and the world surrounding it is perfect, state of the art planning algorithms could generate feasible trajectories that a robot could track through a stiff pre-tuned controllers with high precision. Unfortunately, robots' perception systems are often noisy and unreliable for stiff controllers to interact with the environment, usually leading to a catastrophic failures outside of a well controlled and predefined environment. These controllers could generate undesired forces when encountered with an early unpredicted contact for example. These challenges limit the capability of a robot to execute tasks or behaviors that a human would naturally carry out without any effort. A natural question arises, how are humans capable of executing such tasks smoothly and effortlessly without any challenges?  


%%%%%%%%%%%%%%%%%%%%%%%%%%%% Human Impedance & Risk Opt. %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Motivation: Sensorimotor Impedance, Optimal Feedback \& Risk Awareness}


\quad It was suggested by Burdet \cite{burdet2001central} that humans use impedance modulation, i.e. regulating the relationship between forces and motions  in order to stabilize unstable dynamics of an arm subject to external forces. To achieve this, a set of users were given a robotic manipulator to drive between two points subject to an external divergent force field so that the external force would depend on the direction of the motion. The stiffness of the users' muscles were studied during and after the learning process. It turns out that the geometry and magnitude of the impedance changes between the beginning of the learning process and the time a user masters accomplishing the task. Later studies by Lee et. al. \cite{lee2014time} and \cite{lee2016summary} attempt to study and quantify the mechanical impedance during walking for humans. A wearable robot is used along with linear identification techniques to provide remarkably detailed time varying impedance profiles  during the multiple phases of human locomotion. These profiles clearly indicate pre-tuning of the ankle impedance through the nervous system.  

Liu and Todorov \cite{liu2007evidence} argue that the sensorimotor commands are a result of an optimal feedback control mechanism that controls a trade-off between accuracy and stability. Eventually the authors suggest that the flexibility of the sensorimotor control commands is due to a control law based on the optimization of composite cost functions. The authors of \cite{nagengast2010risk} took this work a step further and proposed using risk sensitive optimal control to model human motor behavior in the face of uncertainty. During experiments, human test subjects would change their control decisions in a risk averse way in the face of increased uncertainty, suggesting that a risk sensitive control approach is more appropriate. In their later work \cite{nagengast2011risk} the trade-off between the mean and the variance (variability) in computational sensorimotor control models was studied, where subjects reportedly show a risk sensitive behavior. That is, motor commands are not a function of a certain reward only, but also subject to its variability.
Various models of risk and how they relate to sensorimotor commands were discussed in \cite{braun2011risk}. Interestingly, Orban \cite{orban2011representations} describes uncertainty in sensorimotor control through a Bayesian framework and characterizes four different types of uncertainties that must be accounted for. These classifications are listed below. 

\begin{itemize}
    \item Motor noise: produces deviations from the control commands, \textbf{a process noise}.
    \item State uncertainty: a result of the imperfections in perception, \textbf{a measurement noise}. 
    \item Parameter uncertainty: characteristics of a task or model parameters are unknown. 
    \item Structural uncertainty: uncertainty at the equations of motion themselves.
\end{itemize}

\noindent The work presented throughout this document will assume the knowledge of the equations of motion while trying to study the effect of the remaining classified uncertainties on the robot control policies generated through optimal control methods. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%% Multi-Contact Robot Dynamics %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multi-Contact Robot Dynamics}


Robots interacting with the environment are usually made from kinematic chains of bodies or links that are interconnected to each other through revolute and prismatic joints as shown in fig. \ref{fig:basic_terminology}. Assuming that the links are rigid bodies will lead to a small number of relatively simply differential equations describing the motion of the robot. As Stewart explains \cite{stewart2000rigid}, modeling elastic bodies in contact with rigid surfaces and subject to Coulomb friction is a computationally complex problem, where the theory is not completely developed even for linearly inelastic bodies. To allow locomotion, one of the links of the robot is designated as the free floating base, and is usually associated with an extra 6 degrees of freedom that are added to the robot model, typically as an $SE(3)$ element \cite{sola2018micro}. This joint is usually unactuated, leading to an underactuated mechanical system. A complete framework for modeling such robots is provided in \cite{murray2017mathematical} while efficiently computing these models through numerical algorithms is presented in \cite{featherstone2014rigid}. The details of this framework are out of the scope of this text. 

\begin{figure}[h]\label{fig:basic_terminology}
\centering
  \includegraphics[width=.8\linewidth]{figures/chapter01/basic_terminology_pdf.pdf}
  \caption{Articulated Kinematic Chain Robot with a Free Floating Base}
  \label{fig:basic_terminology}
\end{figure}

Under the rigid body assumption, the set of differential equations governing the robot motion in multi-contact scenarios are given in eqn. \eqref{eqn:robot_dynamics}. 


\begin{align}
\label{eqn:robot_dynamics}
    M\left(q\right) \dot{v} + h\left(q,v\right)  = S^T \tau + J\left(q\right)^T \lambda_{ext} 
\end{align}

\noindent Where $M\left(q\right)$ is the inertia matrix, $h\left(q,\dot{q}\right)$ is the vector combining the Coriolis and gravity forces.
, $S^T$ is the selection matrix mapping the controls of the actauted joints to the full acceleration vector $\dot{v}$, and $J\left(q\right)^T$ is the transpose of jacobian matrix which maps the contact forces from the contact space to the robot joint space. The dependency on $q$ \& $v$ will be omitted for the remaining of the text. It is also import to define the relevant elements of the equations of motion, their dimensions and the manifolds they live in as described below, 

\footnotesize
\begin{align*}
&nj &&:\quad number\ of\ actuated\ joints \nonumber\\  
&nc &&:\quad number\ of\ active\ contacts \nonumber \\
&nq = nj + 7 &&:\quad configuration \ vector\ size \ including\ quaternions \nonumber\\ 
&nv = nj + 6 &&:\quad dimension \ of \ tangent \ space \nonumber \\ 
&\tau \in R^m &&: \quad control\ inputs \nonumber \\ 
&q \in \mathcal{Q} \subseteq SE\left(3\right)\times R^{nj} &&: \quad element\ of\ configuration\ space \nonumber \\
&v \in \mathcal{T}_{q}\mathcal{Q} \subseteq R^{nv} &&: \quad element \ of  \ tangent \ space \ at \ q \nonumber \\ 
&\lambda_{ext} \in R^{6\times nc} &&: \quad active\ contact \ wrenches \nonumber 
\end{align*}
\normalsize



\subsection{Impedance Control for Robot Contact Tasks}

\quad In his remarkable work, Hogan \cite{hogan1985impedancepart1} postulated that the dynamic interaction between a robot and the environment must be modulated through an impedance controller, that is a controller that would cause the robot appear as an impedance to the environment. Hogan derived an elegant controller that eliminates the need to solve the inverse kinematics problem is derived in \cite{hogan1985impedancepart2}. Hogan's impedance controller implements a second order dynamic behavior relating different variables of a robot such as a contact point position and the force acting on it.  In order to derive this, the second order dynamic behavior of the end-point of a robot is considered as shown in eqn. \eqref{eqn:impedance_manipulator_dynamics} where $M_c$ is a predefined inertia tensor of the contact point, $p$, $\dot{p}$ and $\Ddot{p}$ are the end-point position, velocity and acceleration respectively.Also, K is the desired stiffness whereas B is the desired damping. The dynamics of the environment is described in eqn. \eqref{eqn:impedance_environment_dynamics} where $\lambda_{c}$ resembles interaction force with the manipulator while $\lambda_{other}$ contains any other forces that could be acting on the environment. Given a controller that could track the desired end-point behavior of the robot, the coupled dynamics of the interacting system are described in eqn. \eqref{eqn:impedance_coupled_dynamics}.  

\begin{align}
    \lambda_c &= K \left(p_0 - p\right) + B \left(\dot{p}_0 - \dot{p}\right) - M_c \Ddot{p} \label{eqn:impedance_manipulator_dynamics}\\ 
    M_e \Ddot{p} &= \lambda_c + \lambda_{other} \label{eqn:impedance_environment_dynamics} \\ 
    \left(M_c + M_e\right)\Ddot{p} &=K \left(p_0 - p\right) + B \left(\dot{p}_0 - \dot{p}\right)+ \lambda_{other} \label{eqn:impedance_coupled_dynamics}
\end{align}

\noindent It is straight forward from this point on to derive the contact space variables $p$, $\dot{p}$ and $\Ddot{p}$ as a function of the robot joint space variables $q$, $v$ and $\dot{v}$, then by using the robot dynamics eqn. \eqref{eqn:robot_dynamics} the joint space controller that computes $\tau$ is easily retrieved. The full derivation of the controller is presented in \cite{hogan1985impedancepart2}. An experimental evaluation of this controller during free motion, contact transition and force execution is presented in \cite{hogan1987stable}.


Following the results presented by Hogan, Park \cite{park2001impedance} used a similar approach to design a bipedal walking controller. The derived controller makes a reasonable assumption about the ankle impedance of a biped robot during a locomotion phase. The leg supporting the base is assumed to be stiff to support the desired motion of the base, whereas that of the swinging foot must be stiff during the first part of the swing phase and switch to an over-damped behavior near the contact location to absorb any unwanted or unpredicted impact forces. The results presented show a biped that is able to handle walking on uneven terrain. A similar approach was used for a quadruped trotting gait in \cite{park2012impedance}. Another application of impedance control is presented in \cite{lee2014dynamics} for the MIT Cheetah, where an impedance controller is shown to be stable at various speeds of a periodic trotting gait. In \cite{boaventura2015model} the authors provide a thorough study on the impedance controller of the HyQ quadruped robot using hydraulic actuators. Their work discusses valuable concepts in impedance control design, such as the effect of the controller bandwidth and the concept of natural velocity feedback on the stability margins of the controllers. Kronander \cite{kronander2016stability} later proved that for the variable impedance control case, the standard stability analysis from linear systems theory is not valid. To solve this problem  a Lyapunov based stability constraint relating the stiffness, its rate of change and the damping was introduced. With the advancement in torque controlled robots, impedance controllers became more popular for tasks including contact interactions. The challenge remains in designing the impedance parameters for a given task. Up till today, impedance controllers rely on trial and error methods to tune the stiffness and damping parameters for a given task. This work seeks to develop methods that optimize impedance profiles for given robotic tasks. 


\subsection{Optimal Feedback Control}
 %%%%%%%%%%%%%%%%%%%  Deterministic Optimal Control  %%%%%%%%%%%%%%%%%%%
\quad Optimal feedback control has many promising aspects that could help approach the presented problem. An optimal control formulation allows to generate behaviors and motions from an abstract task formulation, namely the cost function.  This aligns well with the suggested formulations in \cite{liu2007evidence} and \cite{nagengast2011risk}. Another advantage is computing feedback controllers similar in spirit to an impedance controller in a designated state space. The simplest form of an optimal control algorithm is the well known Linear Quadratic Regulator which can be applied to linear systems with quadratic performance criteria.  However, the robots of interest are generally described through nonlinear dynamics, while the tasks desired could be described through nonlinear cost functions. An algorithm that computes local quadratic approximations of both the dynamics and the cost functions then iteratively solves the deterministic optimal control problem was introduced by Mayne \cite{mayne1966second}, this algorithm is commonly known as the Differential Dynamic Programming \textit{DDP} Algorithm.  


Li \cite{li2004iterative} introduced an iterative linear quadratic \textit{iLQR} algorithm, which uses a first order approximation of the dynamics instead of a second order approximation. This algorithm is used to compute energy optimal motions for a musculo-skeletal arm model, however no tasks involving contact interactions were presented. Sideris \cite{sideris2005efficient} provided an in-depth analysis of the algorithm and showed that the search direction computed at each iteration is a descent direction for the optimization problem. He also demonstrated the results on a one dimensional hopping robot model, a task that naturally includes impacts. Tassa  \cite{tassa2012synthesis} formulated and solved an optimal control problem using \textit{DDP} to generate walking trajectories. A complementarity based smooth contact model was used, this allowed for the computation of the gradients and hessians needed for the optimization algorithm. An extension of this work was presented in \cite{tassa2014control}. All the variations of \textit{DDP} presented show  optimistic results of the capabilities of such algorithms to generate dynamically consistent trajectories to fulfill a predefined tasks but the results are not suited for real world applications due to the smoothing assumptions and relaxations introduced in order for the solvers to converge. Another reason is the computation time that cannot be accomplished under real time constraints. 


A real world application appears in \cite{feng20133d} where an \textit{iLQR} algorithm is applied to a reduced inverted pendulum walking model to solve a biped stepping problem in a model predictive control fashion. The desired feet and center of mass trajectories are then assigned as tasks to a QP based inverse dynamics solver which acts as the whole body controller for the full robot. The first implementation of a full state optimal feedback controller is presented for balancing in \cite{mason2014full} and for walking in \cite{mason2016balancing}, linearizations of predefined contact modes are derived, then an LQR controller is used for feedback control on the robot. The issue of control bandwidth was introduced in \cite{grandia2019frequency} where the authors introduce a frequency dependent control term that allows the optimizer to account for the control bandwidth of the actual system, producing smooth control signals. This work was then extended in \cite{grandia2019feedback} to optimize a reduced model that includes base dynamics and contact forces of the quadruped robot ANYMAL. It turns out that the feedback gains computed through deterministic optimal control formulations are too aggressive in scenarios with uncertainty, leading to instabilities in the system. Unfortunately this is always the case as process and measurement noise will always exist in robotics.  

 %%%%%%%%%%%%%%%%%%%  Stochastic Optimal Control  %%%%%%%%%%%%%%%%%%% 
 In \cite{todorov2005generalized}  Todorov added multiplicative process noise that violates the certainty equivalence principle, this change in the problem formulation leads to control policies that are dependent on the process noise. Another way to break the certainty equivalence principle was first introduced by \cite{jacobson1973optimal} for linear systems and later extended to a nonlinear iterative version by Farshidian in \cite{farshidian2015risk}. The main idea behind the iterative Linear Exponential Quadratic algorithm is to solve the optimal control problem for an exponential transformation of the original function. For the case where the noise is assumed to be gaussian, it turns out the solution is a function of both the expectation and variance of the cost function. This formally introduces a controller that could obtain risk neutral, risk sensitive and risk seeking behaviors.  Medina \cite{medina2018considering} used the exponential cost transformation with process noise to perform manipulation tasks through a model predictive control scheme. The stochastic optimal control problem formulation was extended to accommodate for measurement uncertainty in \cite{ponton2016role} where the system dynamics are extended with that of an Extended Kalman filter. A stochastic optimal control algorithm that accounts for higher order statistics of both process and measurement models is the most appealing for designing impedance controllers that bring us closer to human sensorimotor performance. 

==> sections/backup/optimal_control.tex <==
\section{iterative Stochastic Optimal Control}
% Given system dynamics described by the stochastic differential equation 
% \begin{align}
%     dx_t = f\left(x_t,u_t\right) dt + F\left(x_t,u_t\right) d\omega_t
% \end{align}
\textcolor{red}{Everything in this section needs cleaning up}
We are interested in a class of finite horizon stochastic optimal control problems that can be expressed as 

\begin{align}
    \mathcal{J}^{*}\  &=\quad \min_{\pi\left(x_t\right)}\quad   \Psi_{\pi\left(x_t\right)}^{\sigma} \left[\mathcal{L}\left(x,\pi\left(x\right)\right)\right]   \label{eqn:stoch_ocp_cost}\\
    s.t. \quad & \quad  dx_t = f\left(x_t,u_t\right) dt + F\left(x_t,u_t\right) d\omega_t \label{eqn:sde} \\ 
    where \quad& \mathcal{L}\left(x,\pi\left(x\right)\right) = \sum_{t=0}^N l_t\left(x_t,\pi\left(x_t\right),t\right) \\
    &\Psi_{\pi\left(x_t\right)}^{\sigma} \left[f\right] = \frac{1}{\sigma} \log\left(\mathbf{E}\left[\exp{\left(\sigma f\right)}\right] \right)
\end{align}

\noindent $\mathbf{E}\left[\boldsymbol{\cdot} \right]$ is the expectation, taking a first order approximation of our objective function \eqref{eqn:stoch_ocp_cost} gives

\begin{align}
    \Psi_{\pi}^{\sigma} \left[\mathcal{L}\left(x,\pi\right)\right] \approx \mathbf{E}_{\pi}\left[\mathcal{L}\left(x,\pi\right)\right] + \sigma \mathbf{Var}\left[\mathcal{L}\left(x,\pi\right)\right]
\end{align}

\noindent where we will call $\sigma$ the sensitivity parameter. Having a positive sensitivity parameter $\sigma > 0$ means that the higher the variance the higher the cost, thus an optimizer to solve this problem can achieve a lower cost by finding a low variance solution. It was shown in \cite{jacobson1973optimal} that as $\sigma \to + \infty$ the solution converges to that of $H^\infty$ control, a commonly used method in robust control. For the case where  $sigma < 0$,  the higher the variance the lower the cost is, hence an optimizer would prefer a risk seeking behavior, not a very common setting in robotics and control applications, used for exploration in \cite{bechtle2019curious}. In the limit as $\sigma \to 0$ the optimal solution converges to that of minimizing the expectation only, also known as risk neutral control. \cite{dvijotham2012unifying} provides a unified theory on the control of these problems. 

\subsection{Bellman's Principle}
The solution to the finite horizon stochastic optimal control problem can be obtained recursively using Bellman's principle for the risk sensitive problem  \cite{marcus1997risk} defined above, start by defining the value function 

\begin{align}
    v_{t}^{*}\left(x_t\right) = \min_{u_t \in \mathcal{U}} \bigg\{l_t\left(x_t,u_t,t\right) + \Psi_{\pi\left(x_t\right)}^{\sigma} \left[v_{t+1}^{*}\left(x_{t+1}\right)\right] \bigg\}
\end{align}
\noindent This problem is a functional optimization problem, generally intractable as it requires searching the entire state and controls spaces $\mathcal{X},\ \mathcal{U}$. Conservative approximations are generally made to reduce the problem to a tractable one. The most common approximation is restricting the functional space to a linear functions in the states $ \pi\left(x\right) = \tau + K \delta x $. 


\subsection{Risk Neutral Control}
The simplest form of the risk neutral problem is the Linear Quadratic Regulator $LQR$, due to the additive nature of the noise $\omega_t \sim \mathcal{N}\left(0, \Omega \right)$ , the solution is equivalent to the deterministic solution, this is known as the Certainty Equivalent Principle.   

\begin{align}
    dx_t &= \left(Ax_t + Bu_t\right)dt + d\omega_t \\
    \mathcal{L} &= \sum_{t=0}^N x_t^T Q x_t + u_t^T R u_t
\end{align}

\noindent An extension to nonlinear dynamics with nonlinear cost functions was introduced by Mayne \cite{mayne1966second}. A quadratic approximation of the system dynamics and cost function are computed along a nominal state and control trajectories denoted $X^n=\{x^n_0, x^n_1, ..., x^n_N\} , \ U^n=\{u^n_0, u^n_1, ..., u^n_{N-1}\}$  

\begin{align}
    \delta x_t = x_t - x^n_t, \quad \quad \delta u_t = u_t - u^n_t
\end{align}
\noindent A simpler version includes a linear approximation of the dynamics and a quadratic approximation of the cost function \cite{li2004iterative}, the system is approximated as follows 

\begin{align}
    \delta x_{t+1} =& A_t \delta x_t + B_t \delta u_t \\  
    where \quad A_t =& \frac{\partial f}{\partial x}\bigg\vert_{x^n_t,u^n_t} \quad B_t = \frac{\partial f}{\partial u}\bigg\vert_{x^n_t,u^n_t} \nonumber \\
    \mathcal{L}\left(\delta x_t, \delta u_t\right) =& l_N\left(\delta x_N\right) + \sum_{t=0}^{N-1} l_t\left(\delta x_t, \delta u_t\right) \\ 
    l_t\left(\delta x_t, \delta u_t\right) =& \delta x_t^T Q_t \delta x_t + \delta x_t^T q_t + q_t^0 \\
    &+ \delta u_t^T R_t \delta u_t + \delta u_t^T r_t + r_t^0  \nonumber 
\end{align}

\noindent Assuming additive gaussian noise with zero mean, the certainty equivalence principle still holds, the value function is approximated quadratically and the linear control policy is obtained. In \cite{todorov2005generalized} gaussian process noise of multiplicative nature is considered. Under such an assumption, the certainty equivalence principle doesn't hold anymore, this results in a more conservative control policy.  

\subsection{Risk Sensitive Control}
For a linear system with exponential of quadratic cost, Jacobson \cite{jacobson1973optimal} provides a solution for the optimal control problem both in continuous and discrete time. Farshidian \cite{farshidian2015risk} extended the results to non-linear systems where the solution is computed iteratively around a given trajectory. In order to include measurement uncertainty, \cite{speyer1974optimization} suggested a state that grows at each time step to include the entire observed state history. Ponton \cite{ponton2016role} suggested that doubling the size of the state vector to include the dynamics of an Extended Kalman Filter eliminates the need for a growing state vector that includes  the entire state history. 


\begin{align}
    dy_t = h\left(x_t,u_t\right) dt + H\left(x_t,u_t\right)d\gamma   
 \end{align}

\noindent Where $\gamma_t \sim \mathcal{N}\left(0, \Gamma \right)$ , also a quadratic approximation of the cost function can be constructed. In order to account for measurement uncertainty, the system dynamics are extended by the dynamics of an Extended Kalman Filter, given by 

\begin{align}
    \begin{bmatrix} d\left(\delta x_t\right) \\ d\left(\delta \hat{x}_t\right) \end{bmatrix} =& \begin{bmatrix}A_t\delta x_t + B_t \delta u_t \\ A_t\delta x_t + B_t \delta u_t + K_t F_t \left(\delta x_t - \delta \hat{x}_t\right) \end{bmatrix}dt \\ & \quad + \begin{bmatrix} C_t & 0 \nonumber \\ 0 & K_t D_t \end{bmatrix} \begin{bmatrix}d\omega_t \\ d\gamma_t \end{bmatrix}
\end{align}
 \noindent The estimator gains are computed during the forward pass and fixed for the backwards pass. Control law turns out  to be a function of both the state and measurement uncertainty. 

==> sections/backup/problem_definition.tex <==
\section{Multi-Contact Optimal Control Problem}

 Only actual optimized feedback running on a robot that I know of is \cite{mason2014full},\cite{mason2016balancing} and \cite{grandia2019frequency}, \cite{grandia2019feedback}. \cite{mason2014full} and \cite{mason2016balancing} use limited number of linearizaions, solves the LQR and switches between them.  While both \cite{grandia2019frequency} and \cite{grandia2019feedback} use a simplified model of the dynamics that accounts only for the dynamics of the base and the kinematics of the legs, this might be valid for a quadruped, but misses significant effects due to feet swinging in a biped or a manipulator.  

\subsection{System Dynamics with Rigid Contact}

here we define the control problem, contact model used for optimization is similar in spirit to what is introduced in \cite{mastalli2019crocoddyl}. Robot dynamics in multi-contact scenario can be described using 

\begin{align}
\label{eqn:robot_dynamics}
    M\left(q\right) \Ddot{q} + h\left(q,\dot{q}\right)  = S^T \tau + J\left(q\right)^T \lambda_{ext} 
\end{align}

\noindent where, 
\footnotesize
\begin{align*}
&nj &&:\quad number\ of\ actuated\ joints \nonumber\\  
&nc &&:\quad number\ of\ active\ contacts \nonumber \\
&nq = nj + 7 &&:\quad dimension \ of \ configuration \ space \nonumber\\ 
&nv = nj + 6 &&:\quad dimension \ of \ tangent \ space \nonumber \\ 
&\tau \in R^m &&: \quad control\ inputs \nonumber \\ 
&q \in \mathcal{Q} \subseteq SE\left(3\right)\times R^{nj} &&: \quad element\ of\ configuration\ space \nonumber \\
&\dot{q} \in \mathcal{T}_{q}\mathcal{Q} \subseteq R^{nv} &&: \quad element \ of  \ tangent \ space \ at \ q \nonumber \\ 
&\lambda_{ext} \in R^{6\times nc} &&: \quad active\ contact \ wrenches \nonumber 
\end{align*}
\normalsize

\noindent $M\left(q\right)$ is the inertial matrix, $h\left(q,\dot{q}\right)$ is the vector combining the Coriolis acceleration and gravity vector, $S^T$ is the selection matrix mapping the controls to the actauted states, and $J\left(q\right)$ is the jacobian matrix. The dependency on $q$ \& $\dot{q}$ will be omitted for the remaining of the text. A rigid contact model is used to model the contact forces such that the velocity and acceleration of the contact points is zero 

\begin{align}
    \dot{x} &= J \dot{q} = 0 \\
    \Ddot{x} &= \dot{J}\dot{q} + J \Ddot{q} = 0
\end{align}

\noindent In order to resolve the contact forces during integration, the robot dynamics \eqref{eqn:robot_dynamics} is projected to the contact space using $\left(J M^{-1}J^T\right)^{-1} J M^{-1} = \Lambda  J M^{-1} $ to result in 

\begin{align}
 \lambda =   -\Lambda \dot{J}\dot{q} + \Lambda J M^{-1} h - \Lambda J M^{-1} S^T \tau 
\end{align}

\noindent This allows to compute the contact forces satisfying the constraints given $q,\ \dot{q},\&\ \tau$, once $\lambda$ is obtained, the robot accelerations $\Ddot{q}$ can then be computed from  \eqref{eqn:robot_dynamics}  and integrated twice to complete the forward pass of the iterative control algorithms, namely DDP and Risk Sensitive.

\noindent Now we can define the state vector as $x=\left[q, \dot{q}\right]\in \mathcal{X}$ and the motion vector $dx=\left[\dot{q}, \Ddot{q}\right] \in \mathcal{T}_{x}\mathcal{X}$. The first order system dynamics can then be defined as 

\begin{align}
    x_{t+1} = f_t\left(x_t,u_t\right) = x_t \oplus dx_t = x_t \circ exp\left(dx_t\right)
\end{align}

\noindent $f_t\left(x_t,u_t\right)$ represents the drift coefficient $f\left(x,u\right)$ in the stochastic differential equation presented in \eqref{eqn:sde} and $\circ$ represents the group composition operation. 

\subsection{Multi-Contact Optimization}

In order to handle switching in contacts, thus varying dimensions of the contact space, the multi-contact optimal control problem is defined 

\begin{align}
     \min_{\delta X,\delta U}\quad &l_N\left(\delta x_N\right) + \sum_{k=0}^{K} \sum_{t=0}^{T} l_t\left(\delta x_t, \delta u_t\right) %\\ 
\end{align}

\noindent where $K$ is the number of contact switches along along the trajectory and $T$ is the horizon of each phase, this clearly means that contact switches and timings have to be pre-specified by the user. The pros of such approach is that it transforms the non-smooth switches in the contacts to solving the ocp on completely smooth intervals. The contact switches are handled through the switching costs and dynamics.

\subsection{Friction Cone as A Soft Constraint}
Since the rigid contact model doesn't guarantee the unilateral nature of the contact forces, the friction cone is implemented as a soft constraint in the cost function, one possible way is using relaxed barrier functions \cite{hauser2006barrier}, a simpler approximation is used in \cite{mastalli2019crocoddyl} 

\begin{align}
    \sqrt{\lambda_x^2 + \lambda_y^2} &\leq \mu \lambda_z 
\end{align}

\noindent A linear inner approximation of the cone is used to write the cone as $ A \lambda + b \leq 0 $ once this constraint is violated, the cost function activates to penalize the violation. 

==> sections/backup/risk_sensitive.tex <==
\section{risk sensitive optimal control}
Risk sensitive is a form of optimal control that takes into account the uncertainty, breaking away from certainty equivalence principle.
\subsection{Iterative Linear Exponential Gaussian}
\cite{jacobson1973optimal}, \cite{whittle1986hamiltonian}, \cite{dvijotham2012unifying}, \cite{farshidian2015risk},  \cite{medina2018considering}, \cite{bechtle2019curious}

\noindent From Farbod \cite{farshidian2015risk}, the HJB for risk sensitive with process noise 
\begin{align}
-\partial_t \Psi =  \min_u  \{& L +\nabla_x \Psi^T m + \frac{1}{2} Tr\left[\nabla_{xx} \Psi M M^T\right] \nonumber \\ &+ \frac{\sigma}{2} \nabla_x \Psi^T M M^T \nabla_x \Psi \}
\end{align}
\noindent Taking out the last term recovers the usual stochastic HJB, the risk sensitive term is the last one. 
\subsection{Measurement Uncertainty}
It is important to account for uncertainty \cite{schaal2010learning}. Overall result, measurement uncertainty (compliant) has the opposite effect of process uncertainty (stiff), \cite{speyer1974optimization}, \cite{james1994risk},\cite{ponton2016role}

\begin{align}
    dx &= m\left(x,u\right) dt + M\left(x,u\right) d\omega \\
    dy &= n\left(x,u\right) dt + N\left(x,u\right) d\gamma
\end{align}

The cost is given by 
\begin{align}
    \mathcal{J}^{\pi}\left(x,t\right) &= \phi_f \left(x_{t_f}\right) + \int_{t}^{t_f} L\left(x_t,u_t,t\right) dt \\
    \mathbf{J} &= \min_{\pi} \mathbb{E}\{ \mathbf{exp} \left[\sigma \mathcal{J}^{\pi}\right]\}
\end{align}

\textcolor{blue}{$\mathbf{J}$  is therefore the risk- sensitive cost and corresponds to the moment generating function, an alternative specification of the probability distribution of the random variable $\mathcal{J}^{\pi}$}.
 
 \noindent Farshidian \cite{farshidian2015risk}, shows that the cumulant generating function of $\mathbf{J}$  can be written as a linear combination of the moments of $\mathcal{J}^{\pi}$. 
 \begin{align}
     \frac{1}{\sigma} \log \left[\mathbf{J}\right] = \mu_1 \left[ \mathcal{J}^{\pi}\right] + \frac{\sigma}{2} \mu_2 \left[\sigma \mathcal{J}^{\pi}\right] + \frac{\sigma^2}{6} \mu_3 \left[\sigma \mathcal{J}^{\pi}\right] + ...
 \end{align}
 \noindent \textcolor{blue}{Depending on $\sigma$, there will be a compromise between increasing control effort and narrowing confidence intervals}. Ponton \cite{ponton2016role} derives a locally optimal feedback control law by reformulating the problem to include measurement noise. Starts by following a common approach in iterative optimal control \cite{mayne1966second}, \cite{todorov2005generalized} and construct a linearization around the nominal trajectory. 
 
 \begin{align}
     \delta x_t &= x_t - x_t^n \\
     \delta u_t &= u_t - u_t^n \\ 
     d\left(\delta x_t\right) &= \left(A_t\delta x_t + B_t \delta u_t\right)dt + C_t d\omega_t \\ 
     d\left(\delta y_t\right) &= \left(F_t\delta x_t + E_t \delta u_t\right)dt + D_t d\gamma_t 
 \end{align}

Also a quadratic approximation of the cost function can be constructed. In order to account for measurement uncertainty, the system dynamics are extended by the dynamics of the estimator, given by 

\begin{align}
    \begin{bmatrix} d\left(\delta x_t\right) \\ d\left(\delta \hat{x}_t\right) \end{bmatrix} =& \begin{bmatrix}A_t\delta x_t + B_t \delta u_t \\ A_t\delta x_t + B_t \delta u_t + K_t F_t \left(\delta x_t - \delta \hat{x}_t\right) \end{bmatrix}dt \\ &+ \begin{bmatrix} C_t & 0 \nonumber \\ 0 & K_t D_t \end{bmatrix} \begin{bmatrix}d\omega_t \\ d\gamma_t \end{bmatrix}
\end{align}
 \noindent The estimator gains are computed during the forward pass and fixed for the backwards pass. In order to compute the estimator gain, minimize the square error of the dynamics given by 
 
 \begin{align}
     d\left(\delta e_t \right) &=  d\left(\delta x_t \right) - d\left(\delta \hat{x}_t \right) \nonumber \\ 
     &= A_t \delta e_t dt + C_t d\omega_t - K_t \left[d\left(\delta y_t \right) - d\left(\delta \hat{y}_t \right)\right] \nonumber \\ 
     &= \left(A_t - K_t F_t\right)\delta e_t dt + C_t d\omega_t - K_t D_t d\gamma_t 
 \end{align}
 
 \noindent The uncertainty in the error dynamics is given by 
 
 \begin{align}
     \dot{\Sigma}_t^e &= \mathbb{E} \{d\left(\delta e_t \right) d\left(\delta e_t \right)^T\} \nonumber \\ 
     &= \left(A_t - K_t F_t\right)\Sigma_t^e + \Sigma_t^e \left(A_t - K_t F_t\right)^T \nonumber \\ & \ \ + K_tD_t\Gamma_t D_t^T K_t^T + C_t \Omega_t C_t^T  \\ 
     K_t &= \Sigma_t^e F_t^T \left(D_t\Gamma_t D_t^T\right)^{-1}
 \end{align}
 
 \noindent Let's skip the value function derivation and optimization and examine the resulting control law 
 \begin{align}
     H_t &= in \  appendix \ ? \\
     g_t &= in \  appendix \ ? \\
     G_t^x &= in \  appendix \ ?  \\ 
     G_t^{\hat{x}} &= in \  appendix \ ?  \\ 
     \delta u_t &= - H_t^{-1} g_t - H_t^{-1} \left(G_t^x + G_t^{\hat{x}}\right) \delta x_t  
 \end{align}
 
 \begin{itemize}
     \item \textcolor{red}{Feedforward and feedback terms are different from DDP, why does the feedforward control turnout to be the same for both solvers?} \\
     \item \textcolor{red}{How does this feedback law compare to that of iLQR or DDP?}
 \end{itemize}
 
 \noindent  The optimal control law is substituted back into the value function, it has negative terms that contribute to reducing the cost. \textcolor{blue}{Even if the measurement noise is set to zero, the control law is still not equivalent to the one found in} \cite{farshidian2015risk}. \textcolor{red}{Is this due to the assumption made to depend completely on estimated state statistics during the optimization step?} 
 
